Polynomial-Time Algorithms for Submodular Laplacian Systems

Let $G=(V,E)$ be an undirected graph, $L_G\in \mathbb{R}^{V \times V}$ be the associated Laplacian matrix, and $b \in \mathbb{R}^V$ be a vector. Solving the Laplacian system $L_G x = b$ has numerous applications in theoretical computer science, machine learning, and network analysis. Recently, the notion of the Laplacian operator $L_F:\mathbb{R}^V \to 2^{\mathbb{R}^V}$ for a submodular transformation $F:2^V \to \mathbb{R}_+^E$ was introduced, which can handle undirected graphs, directed graphs, hypergraphs, and joint distributions in a unified manner. In this study, we show that the submodular Laplacian system $L_F( x) \ni b$ can be solved in polynomial time. Furthermore, we also prove that even when the submodular Laplacian system has no solution, we can solve its regression form in polynomial time. Finally, we discuss potential applications of submodular Laplacian systems in machine learning and network analysis.

==> digraph.tex <==
%!TEX root=./main.tex

\section{Directed Graphs}\label{sec:digraphs}

\subsection{Exact solution}

Let $G=(V,E)$ be a directed graph and $\bmb \in \bbR^V$ be a vector.
In this section, we show how to solve $L_G(\bmx) = \bmb$.

Let us consider the following optimization problem:
\begin{align}
  \begin{array}{lll}
    \text{minimize} & \displaystyle D_{G,\bmb}(\bmx) := \frac{1}{2}\sum_{uv \in E}\max(\bmx(u)-\bmx(v),0)^2-\sum_{v \in V}\bmb(v)\bmx(v).
  \end{array}\label{eq:digraph-primal}
\end{align}

\begin{lemma}
    Suppose that \eqref{eq:digraph-primal} is bounded.
    Then \eqref{eq:digraph-primal} has an optimal solution and an optimal solution $\bmx^*$ \eqref{eq:digraph-primal} satisfies $L_G(\bmx^*) = \bmb$.
\end{lemma}
\begin{proof}
    First note that the objective is continuously differentiable.
    More precisely,
    \begin{align*}
        \frac{\partial D}{\partial \bmx(u)}
        &= \sum_{uv \in E} \max(\bmx(u) - \bmx(v), 0) - \sum_{vu \in E}\max(\bmx(v) - \bmx(u), 0) - \bmb(u)  \\
        &= L_G(\bmx)(u) - \bmb(u).
    \end{align*}
    Therefore the first order optimality condition is $L_G(\bmx) = \bmb$.
\end{proof}
\ynote{What's the time complexity for directly solving~\eqref{eq:digraph-primal}?}
\tnote{I suggest solving \eqref{eq:energy-minimization} instead, since \eqref{eq:energy-minimization} has more rich combinatorial structure.}

\subsection{Energy Minimization Interpretation}
The dual problem of \eqref{eq:digraph-primal} is the following energy-minimization problem:
\begin{align}
  \begin{array}{lll}
  \text{minimize} & \displaystyle \frac{1}{2}\sum_{e\in E}\bmphi(e)^2\\
  \text{subject to}& \displaystyle \sum_{vw\in E}\bmphi(vw) - \sum_{uv \in E} \bmphi(uv) = \bmb(v) & (v \in V) \\
  & \bmphi(e) \geq 0 & (e \in E)
  \end{array}
  \label{eq:energy-minimization}
\end{align}

To see this, for fixed $\bmx \in \bbR^V$ and $\bmy \in \bbR^E$ with $\bmy \leq \bmzero$, observe that the Lagrange relaxation of~\eqref{eq:energy-minimization} is the following:
\begin{align}
  \begin{array}{ll}
  \text{minimize } & P_{G,\bmb}(\bmphi,\bmx,\bmy)  \\
  \text{where } & P_{G,\bmb}(\bmphi,\bmx,\bmy) :=
\\
  &    \displaystyle  \frac{1}{2}\sum_{e\in E}\bmphi(e)^2 - \sum_{v \in V} \bmx(v) \Bigl(\sum_{vw\in E}\bmphi(vw) - \sum_{uv \in E} \bmphi(uv)  - \bmb(v) \Bigr) - \sum_{e \in E}\bmy(e) \bmphi(e).
  \end{array}
  \label{eq:lagrange-primal}
\end{align}

We now consider maximizing~\eqref{eq:lagrange-primal} over $\bmx \in \bbR^V$ and $\bmy \in \bbR^E$ with $\bmy \geq \bmzero$.
First, we have
\begin{align}\label{eq:digraph-saddle-cond}
  \frac{\partial P_{G,\bmb}(\bmphi,\bmx,\bmy)}{\partial \bmphi(uv)} = \bmphi(uv) + \bmx(v) - \bmx(u) - \bmy(uv).
\end{align}
Under the condition that $\frac{\partial P_{G,\bmb}(\bmphi,\bmx,\bmy)}{\partial \bmphi(e)} = 0$ for every $e \in E$, we obtain
\begin{align*}
  P_{G,\bmb}(\bmphi,\bmx,\bmy)
  & = \sum_{v \in V}\bmb(v)\bmx(v) -\frac{1}{2}\sum_{uv \in E}\bmphi(e)^2 \\
  & = \sum_{v \in V}\bmb(v)\bmx(v) -\frac{1}{2}\sum_{uv \in E}(\bmx(u)-\bmx(v)+\bmy(uv) )^2.
\end{align*}
To maximize $P_{G,\bmb}(\bmphi,\bmx,\bmy)$, we should choose $\bmy(uv) = \bmx(v)-\bmx(u)$ if $\bmx(u) - \bmx(v) \leq 0$ and $\bmy(uv) = 0$ otherwise.
Then, we get the following dual problem.
\begin{align*}
    \text{maximize} \sum_{v \in V}\bmb(v)\bmx(v) -\frac{1}{2}\sum_{uv \in E}\max(\bmx(u)-\bmx(v),0)^2,
\end{align*}
which is \eqref{eq:digraph-primal}.
Since \eqref{eq:digraph-primal} is an unconstrained problem, the Slater condition is trivially satisfied.
Thus the strong duality holds.
Furthermore, since the objective in \eqref{eq:energy-minimization} is strictly convex, there exists a unique optimal solution $\bmphi^*$ for \eqref{eq:energy-minimization}.
The energy minization problem~\eqref{eq:energy-minimization} is an instance of \emph{quadratic network flow problem}, which can be solved $O(n^3)$ time.
Once the optimal solution $\bmphi^*$ of \eqref{eq:energy-minimization} is obtained, one can reconstruct a primal optimal solution $\bmx^*$ via linear equation \eqref{eq:digraph-saddle-cond}.

% Then, we have $\bmphi^*(uv) = \max(\bmx^*(u)-\bmx^*(v),0)$ for every $uv \in E$.

% \ynote{show strong duality}

\subsection{Regression}
Let $G=(V,E)$ be a directed graph and $\bmb \in \bbR^V$ be a vector.
In this section, we show how to minimize $\|L_G(\bmx) - \bmb\|_2^2$.

Let $B \subseteq \bbR^V$ be the set of vectors $\bmb$ for which~\eqref{eq:digraph-primal} is bounded (from above).
\begin{lemma}
  The set $B$ is convex.
\end{lemma}
\begin{proof}
  Suppose that~\eqref{eq:digraph-primal} is bounded for $\bmb,\bmb' \in \bbR^V$ but is not bounded for $\bmb'' \in \bbR^V$, which is a convex combination of $\bmb$ and $\bmb'$.
  Then, for arbitrary large number $N$, there exists $\bmx \in \bbR^V$ such that $\caD_{G,\bmb''}(\bmx) \geq N$.
  Also, it is easy to see that $\caD_{G,\bmb''}(\bmx)$ is a convex combination of $\caD_{G,\bmb'}(\bmx)$ and $\caD_{G,\bmb'}(\bmx)$.
  As the choice of $N$ was arbitrary, this means that~\eqref{eq:digraph-primal} on $\bmb$ or $\bmb'$ must be unbounded, which is a contradiction.
\end{proof}


Now, we consider the following problem:
\begin{align}
  \begin{array}{ll}
    \text{minimize}& \|\bmb'-\bmb\|_2^2\\
    \text{subject to} &\bmb' \in B.
  \end{array}\label{eq:digraph-regression}
\end{align}

Note that once we get a solution $\bmb^* \in B$, we can recover $\bmx \in \bbR^V$ such that $L(\bmx) = \bmb^*$.
%\ynote{Under which condition we can solve this problem efficiently? I think just that $B$ is convex is not enough.}


Next, we consider conditions of $\bmb \in \bbR^V$ that makes minimum of $\caD_{G,\bmb}$ is unbounded.
To this end, we fix an ordering $\pi$ of $V$ and consider conditions of $\bmb \in \bbR^V$ that makes the minimum of $\caD_{G,\bmb}$ in the region $\bbR^V_\pi$.
\begin{lemma}\label{lem:digraph-unbounded-in-pi}
  Let $\pi$ be an ordering of $V$.
  Then, $\caD_{G,\bmb}$ is unbounded in the region $\bbR^V_\pi$ if and only if at least one of the following hold:
  \begin{itemize}
  \item There exists $k \in [n]$ such that $\bmb(\set{\pi_1,\ldots,\pi_k}) > 0$ and there is no arc $\pi_i\pi_j$ with $i \in \set{1,\ldots,k}$ and $j \in \set{k+1,\ldots,n}$, or
  \item There exists $\ell \in [n]$ such that $\bmb(\set{\pi_\ell,\ldots,\pi_n}) < 0$ and there is no arc $\pi_i\pi_j$ with $i \in \set{1,\ldots,\ell-1}$ and $j \in \set{\ell,\ldots,n}$.
  \end{itemize}
\end{lemma}
\begin{proof}
  ($\Rightarrow$)
  If $\caD_{G,\bmb}$ is unbounded in the region $\bbR^V_\pi$, there exist $\bmx \in \bbR^V_{\pi}$, $0 \leq k<\ell \leq n+1$ and $\alpha,\beta \in \bbR_+$ with the following property:
  For $\bmv = \alpha\bmone_{\set{1,\ldots,k}} - \beta\bmone_{\set{\ell,\ldots,n}}$, we have $\lim\limits_{t \to \infty}\caD_{G,\bmb}(\bmx + t\bmv) \to -\infty$.
  In particular, this means $\lim\limits_{t \to \infty}\caD_{G,\bmb}(\bmx + t\bmv) - \caD_{G,\bmb}(\bmx) \to -\infty$.
  Then, for any $\bmw_e \in \partial f_e(\bmx)\;(e\in E)$, we have
  \begin{align*}
    \caD_{G,\bmb}(\bmx+t\bmv) - \caD_{G,\bmb}(\bmx)
    & = \frac{1}{2}\sum_{e \in E}\Bigl(\langle \bmw_e,\bmx+t\bmv \rangle^2-\langle \bmw_e,\bmx \rangle^2\Bigr) - \Bigl(\langle\bmb,\bmx+t\bmv\rangle - \langle\bmb,\bmx\rangle\Bigr) \\
    & = \frac{1}{2}\sum_{e \in E}\Bigl(\langle \bmw_e,t\bmv \rangle^2 +\langle \bmw_e,t\bmv \rangle \langle \bmw_e,2\bmx \rangle\Bigr)- \langle\bmb,t\bmv\rangle.
  \end{align*}
  To make this unbounded when $t \to \infty$, we must have $\langle \bmb,\bmv\rangle > 0$ and $\langle\bmw_e,\bmv\rangle=0$ for every $e \in E$.
  Then, we must have
  \begin{itemize}
  \item $\alpha \bmb(\set{\pi_1,\ldots,\pi_k}) - \beta\bmb(\set{\pi_\ell,\ldots,\pi_n}) > 0$
  \item if $\alpha > 0$, there is no arc $\pi_i\pi_j$ with $i \in \set{1,\ldots,k}$ and $j \in \set{k+1,\ldots,n}$
  \item if $\beta > 0$, there is no arc $\pi_i\pi_j$ with $i \in \set{1,\ldots,\ell-1}$ and $j \in \set{\ell,\ldots,n}$.
  \end{itemize}
  These conditions can be simplified to the following
  \begin{itemize}
  \item $\bmb(\set{\pi_1,\ldots,\pi_k}) > 0$ and there is no arc $\pi_i\pi_j$ with $i \in \set{1,\ldots,k}$ and $j \in \set{k+1,\ldots,n}$, or
  \item $\bmb(\set{\pi_\ell,\ldots,\pi_n}) < 0$ and there is no arc $\pi_i\pi_j$ with $i \in \set{1,\ldots,\ell-1}$ and $j \in \set{\ell,\ldots,n}$.
  \end{itemize}

  ($\Leftarrow$) Trivial.
\end{proof}

\begin{corollary}\label{cor:digraph-unbounded-in-pi}
  $\caD_{G,\bmb}$ is unbounded in $\bbR^V$ if and only if there exists a set $S \subseteq V$ that satisfies at least one of the following:
  \begin{itemize}
  \item[(i)] $\bmb(S) > 0$ and there is no arc from $S$ to $V \setminus S$.
  \item[(ii)] $\bmb(S) < 0$ and there is no arc from $V \setminus S$ to $S$.
  \end{itemize}
\end{corollary}
% \begin{proof}
%   $(\Rightarrow)$

%   \ynote{Prove this.}
%   \ynote{Actually, the second condition is equivalent to the first condition if $\bmb \perp \bmone$.}

%   $(\Leftarrow)$
%   Trivial.
% \end{proof}

Now, we give an algorithm that checks the conditions in Corollary~\ref{cor:digraph-unbounded-in-pi}.
First, we create an auxiliary graph $G' = (V',E', \bmc)$,
where $V' = V \cup \set{s,t}$ for newly introduced vertices $s$ and $t$, $E' = E \cup \set{sv \mid v \in V} \cup \set{vt \mid v \in V}$.
For each arc $e \in E$, we set $c(e) = \infty$.
For each $v \in V$, we set $\bmc(sv) = \bmb(v)$ if $\bmb(v) > 0$ and $\bmc(vt) = -\bmb(v)$ if $\bmb(v) < 0$.

Consider an $s$-$t$ minimum cut $S^*$ on $G'$.
Then, $S^*$ is a minimizer of the function
\[
  \sum_{v \in V:\bmb(v)>0}\bmb(v) -\sum_{v \in S:\bmb(v)> 0}\bmb(v)+\sum_{v \in S: \bmb(v) < 0}(-\bmb(v))
  =
  \sum_{v \in V:\bmb(v)>0}\bmb(v) - \bmb(S),
\]
subject to having no arc from $S$ to $V \setminus S$, which maximizes $\bmb(S)$,
Hence, we can check the first condition of Corollary~\ref{cor:digraph-unbounded-in-pi}.

By using a similar auxiliary graph, we can check the second condition of Corollary~\ref{cor:digraph-unbounded-in-pi}.
This means that we can decide whether $\caD_{G,\bmb}$ is unbounded or not for any fixed $\bmb \in \bbR^V$.


From Corollary~\ref{cor:digraph-unbounded-in-pi}, the regression problem can be solved by solving the following:
\begin{align}
  \begin{array}{lll}
    \text{minimize} & \|\bmp\|_2^2 \\
    \text{subject to} & \bmb(S) + \bmp(S) \leq 0 & \forall S \subseteq V, \text{no out-neighbor} \\
    & \bmb(S) + \bmp(S) \geq 0 & \forall S \subseteq V, \text{no in-neighbor} \\
%    & \bmp(V) = 0\\
  \end{array}
  \label{eq:regression2}
\end{align}
Note that $\bmb(V) + \bmp(V)=0$ from the constraints.
Then, we can further simplify~\eqref{eq:regression2} as follows by considering $V-S$ for $S \subseteq V$ with no in-neighbor.
\begin{align}
  \begin{array}{lll}
    \text{minimize} & \|\bmp\|_2^2 \\
    \text{subject to} & \bmp(S) \leq -\bmb(S) & \forall S \subseteq V, \text{no out-neighbor}.
  \end{array}
  \label{eq:regression3}
\end{align}


% \tnote{What does $\bmx$ mean here? Is it intended for $\bmx = \bmb - \bmb'$ or a solution for $\min \| L(\bmx) - \bmb \|^2$?}
% \ynote{$\bmp$ is intended to express $\bmb'-\bmb$.}
% \tnote{Why do we need $x(V) = 0$?}
% \ynote{I guess I was thinking the case the given $\bmb$ is orthogonal to $\bmone$.}
%As we already have the separation oracle for this problem, this problem can be solved in polynomial time by ussing the ellipsoid method.

Let $\ker F = \set{S \subseteq V \mid F(S) = \bmzero}$. Since $\ker F$ forms the distributive lattice, the feasible region of \eqref{eq:regression3} coincides with the submodular polytope $P_\caD(-\bmb)$, where $\caD = \ker F$.
Therefore \eqref{eq:regression3} is the minimum norm problem in $P_\caD(-\bmb)$.
Since we can optimize linear functions over the polytope $P_\caD(-\bmb)$ in polynomial time,  we can use Frank-Wolfe's algorithm for the minimum-norm point problem.
In Appendix~\ref{app:minnorm}, we show that the minimum norm problem in $P_\caD(-\bmb)$ can be reduced to parametric submodular minimization.



==> hypergraph.tex <==
%!TEX root=main.tex

\section{Hypergraphs}

Let $G=(V,E)$ be a hypergraph and $\bmb \in \bbR^V$ be a vector.
Consider the following optimization problem:
\begin{align*}
    \begin{array}{lll}
        \text{minimize} &\displaystyle \sum_{v \in V}\bmb(v) \bmx(v) + \frac{1}{2}\sum_{e \in E}\bmeta(e)^2 \\
        \text{subject to} & \displaystyle \bmx(u) - \bmx(v) \leq \bmeta(e) &  (e \in E, u,v \in e).
    \end{array}
\end{align*}

The Lagrange relaxation is
\begin{align*}
    \begin{array}{lll}
        \text{minimize } & \displaystyle \caE_{G,\bmb}(\bmf,\bmx,\bmeta) := \sum_{v \in V}\bmb(v) \bmx(v) + \frac{1}{2}\sum_{e \in E}\bmeta(e)^2 - \sum_{e \in E} \sum_{u,v \in E} \bmf(e,u,v)(\bmeta(e) - (\bmx(u) - \bmx(v))) \\
        \text{subject to} & \displaystyle \bmf(e,u,v) \geq 0 \quad (e \in E, u,v \in e).
    \end{array}
\end{align*}
We have
\begin{align*}
    \frac{\partial \caE_{G,\bmb}(f,\bmx,\bmeta)}{\partial \bmx(v)} & = \bmb(v) + \sum_{e \in E}\sum_{w \in E}\bmf(e,v,w) - \sum_{e \in E}\sum_{u \in E}\bmf(e,u,v), \\
    \frac{\partial \caE_{G,\bmb}(f,\bmx,\bmeta)}{\partial \bmeta(e)} & = \bmeta(e) - \sum_{u,v \in e}\bmf(e,u,v).
\end{align*}
When these are zero, we have
\begin{align*}
    \caE_{G,\bmb}(\bmf,\bmx,\bmeta) = -\frac{1}{2}\sum_{e \in E}(\sum_{u,v\in e}\bmf(e,u,v))^2.
\end{align*}

For every $e \in E$, we have
\begin{align*}
    \bmx(u) - \bmx(v) \leq \sum_{u,v \in e}\bmf(e,u,v).
\end{align*}

\ynote{I guess by complementary slackness $\bmf(e,u,v) > 0$ if and only if $\bmx(u)-\bmx(v) = \bmeta(e)$, which indicates that the pair $(u,v)$ maximizes the differences $\bmx(u)-\bmx(v)$. This successfully expresses the hypergraph Laplacian. Maybe we can generalize this to general submodular Laplacians...}
